Uncertainty-Aware Deployment of Pre-trained Language-Conditioned Imitation Learning Policies

Large-scale robotic policies trained on data from diverse tasks and robotic platforms hold great promise for enabling general-purpose robots; however, reliable generalization to new environment conditions remains a major challenge. Toward addressing this challenge, we propose a novel approach for uncertainty-aware deployment of pre-trained language-conditioned imitation learning agents. Specifically, we use temperature scaling to calibrate these models and exploit the calibrated model to make uncertainty-aware decisions by aggregating the local information of candidate actions. We implement our approach in simulation using three such pre-trained models, and showcase its potential to significantly enhance task completion rates. The accompanying code is accessible at the link: https://github.com/BobWu1998/uncertainty_quant_all.git

==> tex/extras.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/rvt/ood_uncertainty_rvt.png}
    \vspace{-6pt}
    \caption{Uncertainty Measure for task 'put groceries in cupboard' and its variants}
    \label{fig: ood_uncertainty_rvt}
    \vspace{-12pt}
\end{figure*}
